Quantifying Privacy via Information Density

We examine the relationship between privacy metrics that utilize information density to measure information leakage between a private and a disclosed random variable. Firstly, we prove that bounding the information density from above or below in turn implies a lower or upper bound on the information density, respectively. Using this result, we establish new relationships between local information privacy, asymmetric local information privacy, pointwise maximal leakage and local differential privacy. We further provide applications of these relations to privacy mechanism design. Furthermore, we provide statements showing the equivalence between a lower bound on information density and risk-averse adversaries. More specifically, we prove an equivalence between a guessing framework and a cost-function framework that result in the desired lower bound on the information density.

==> sections/intro_parastoosnotes.tex <==
\begin{itemize}
\item LDP is a symmetric metric that bounds the logarithm of ratio of any two values in the channel transition probability matrix from below and above by $-\epsilon$ and $\epsilon$, respectively.
\item The same symmetric methodology has been applied to LIP. That is, LIP which is also information density is also bounded from below and above by $-\epsilon$ and $\epsilon$. However, LIP is a context-aware (prior-dependent) notion of privacy and it is not a symmetric definition as it is the ratio of posterior to prior distributions. 
\item As shown in the literature, enforcing symmetric bounds can cause degradation in utility, thereby erasing the potential benefit of a context-aware mechanism design. Moreover, since the definition of LIP is not symmetric, a motivation for the lower bound is missing.
\item Two approaches have been pursued in the literature: one is PML which altogether avoids imposing a lower bound on the information density (also referred to as lift) values. The other approach has been asymmetric LIP which imposes different lower and upper bounds on the information density (lift) values, thereby allowing a more degrees of freedom in tradeoff between utility and privacy compared to symmetric LIP.
\end{itemize}

But we know information density (lift) values cannot take any values completely  from other information density (lift) values. For one, probabilities in the ratios have to satisfy basic probability conditions. Such stochastic conditions impose some restriction on how the lower bound and upper on information density (lift) behave in relation to each other. Maybe talk about some obvious relations. 

In this paper we make these relations precise and study how they impact privacy mechanism design. Blah blah.



==> sections/mechdesign_short.tex <==
\label{sec:optmech}
%From the above derivations, we can see that there are $(\epsilon_l,\epsilon_u)$-ALIP guarantees which are implied by $\epsilon_u$-PML. More specifically, for cases in which the lower bound on information density is implied by the upper bound, that is, for $\epsilon_l \leq \epsilon_l(\epsilon_u)$, mechanisms optimal for $\epsilon$-PML are also optimal for $(\epsilon_l,\epsilon_u)$-ALIP, as is shown in the following proposition.

\begin{proposition}
\label{prop:optimalPML}
 Assume $X$ is distributed according to $P_X$. Then, for all $\epsilon_u < \frac{1}{1-p_{\min}}$, the optimal $(\epsilon_l,\epsilon_u)$-ALIP mechanism with $\epsilon_l \geq \epsilon_l(\epsilon_u)$ is given by the mechanism optimal for $\epsilon_u$-PML. 
\end{proposition}
\begin{IEEEproof}
    The proof is by contradiction. Denote the optimal $\epsilon$-PML mechanism as $P_{Y|X}^{*,\epsilon}$. Assume there exists a mechanism $P_{Y|X}^*$ satisfying $(\Tilde{\epsilon},\epsilon)$-ALIP such that $U(P_{Y|X}^*) > U(P_{Y|X}^{*,\epsilon})$. Then, since $(\Tilde{\epsilon},\epsilon)$-ALIP implies $\epsilon$-PML, $P_{Y|X}^{*,\epsilon}$ could not be the optimal PML mechanism, which yields a contradiction, as desired.
\end{IEEEproof}
